LGMCTS: Language-Guided Monte-Carlo Tree Search for Executable Semantic Object Rearrangement

We introduce a novel approach to the executable semantic object rearrangement problem. In this challenge, a robot seeks to create an actionable plan that rearranges objects within a scene according to a pattern dictated by a natural language description. Unlike existing methods such as StructFormer and StructDiffusion, which tackle the issue in two steps by first generating poses and then leveraging a task planner for action plan formulation, our method concurrently addresses pose generation and action planning. We achieve this integration using a Language-Guided Monte-Carlo Tree Search (LGMCTS). Quantitative evaluations are provided on two simulation datasets, and complemented by qualitative tests with a real robot.

==> introduction.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% State the usage robot semantic rearrangment in real-world
\section{INTRODUCTION}
In daily life, tasks like ``Set up the kitchen" require arranging objects according to language cues, an intuitive process for humans but a complex challenge for robots. The semantic rearrangement problem aims to enable robots to reconstruct scenes based on linguistic descriptions. This necessitates the seamless integration of scene understanding, linguistic reasoning, and action planning, involving multiple disciplines such as robotics and natural language processing.

% In daily life, we often need to arrange objects based on verbal instructions or language descriptions. Tasks as simple as ``Set up the kitchen" encapsulate objects' nuanced and complex choreography in relation to their spatial and functional contexts. For humans, such linguistic cues are easily translated into tangible actions. However, for robots, this presents a multifaceted challenge. The semantic rearrangement problem delves into this very complexity. At its core, it seeks to enable a robot to reconstruct a scene based on a linguistic description. This involves the intricate integration of scene understanding, linguistic reasoning, and action planning. Addressing these challenges requires a confluence of robotics, natural language processing, and planning. 

% Explain the difficulty of the problem
Consider the task: ``Set the dinnerware for dinner and place a candle in front of a plate." A robot must identify the items constituting `dinnerware' and their correct arrangement, while also handling real-world constraints like initial object coverings and spatial obstacles. The command introduces two key constraints: 1) `dinnerware' must be arranged appropriately for dinner, and 2) a candle must be placed in front of a plate. This example highlights the problem's complexity.

% Consider this scenario: ``Set the dinnerware for dinner and place a candle in front of a plate". To address this command, a robot must discern what `dinnerware' signifies within the scene and the appropriate arrangement for dinner. Real-world settings introduce physical dependencies; if `dinnerware' implies a knife, fork, and plate, such objects can be initially covered. There could also be obstacles at the plate's intended position. Two constraints emerge from the instruction: 1) the dinnerware must align with a dinner setting, and 2) a candle must be positioned in front of the plate. This example underscores the intricate nature of the challenge.

% Approaches-1: Multi-modality transformer
% StructFormer, VIMA, CLIPPORT
One approach employs a multi-modality transformer~\cite{clip_port, liu2022structformer, vima} to learn the mapping between language and object poses through simulated arrangements and rule-based language descriptions. However, this method has limitations. It assumes that language descriptions map to precise ground-truth poses, which is often unrealistic. It is also less adaptable to free-form linguistic inputs, as it performs best with descriptions similar to its training data.

% One approach to this problem involves employing a multi-modality transformer~\cite{clip_port, liu2022structformer, vima}. By simulating a multitude of arrangement outcomes and accompanying them with language descriptions derived from pre-defined rules, a transformer can learn the inherent mapping between linguistic tokens and the corresponding desired poses. However, this methodology comes with significant constraints. First, it operates on the assumption that a single language description exclusively corresponds to precise ground-truth poses. This is often misaligned with real-world scenarios where language descriptions are more ambiguous, pointing to a region rather than a specific spot. Furthermore, this method is most effective with language descriptions that mirror its training data, proving less adaptable to free-form linguistic inputs.

% Approaches-2: Diffusion Model-based method
% DALLE-E-BOT, StructDiffusion
Recent research employs diffusion models to capture how language tokens map to spatial distributions. DALL-E-Bot~\cite{Dall-e-bot} uses text-to-image to generate target images and derive poses, while StructDiffusion~\cite{struct_diffusion} employs a diffusion model conditioned on language and point-cloud embeddings. Both approaches show promise but have limitations: DALL-E-Bot can be unstable and distracted by extraneous objects, whereas StructDiffusion is constrained to known training patterns and lacks zero-shot adaptability.

% Recognizing that language descriptions often refer to regions or distributions, researchers have recently turned to diffusion models to encapsulate the relationship between language tokens and their associated distribution mappings. DALL-E-Bot~\cite{Dall-e-bot} employs a text-to-image mechanism to generate the target rearrangement image and subsequently derive object poses from it. Conversely, StructDiffusion~\cite{struct_diffusion} constructs a diffusion model designed to generate object poses conditioned on both language and point-cloud embeddings. This approach has demonstrated improved results in addressing semantic rearrangement challenges. However, both methods have their limitations. DALL-E-Bot, while innovative, exhibits instability and is prone to distraction by extraneous objects. StructDiffusion, on the other hand, is limited to the patterns that it has been trained on, lacking the flexibility to accommodate zero-shot pattern compositions.

% Code-as policies
Moreover, recent developments emphasize direct robot control through Large Language Models (LLMs)~\cite{gpt3, llama, llama2} and prompt techniques such as Chain of Thoughts (COT)~\cite{COT}. The `Code-as-policies'~\cite{code-as-policies} approach shows remarkable zero-shot capabilities and could theoretically address the semantic rearrangement problem, leveraging LLMs' strength in pattern comprehension and object selection.

% In recent developments, with the rise of Large Language Models (LLMs)~\cite{gpt3, llama, llama2}  and advanced prompt engineering techniques, such as Chain of Thoughts (COT)~\cite{COT}, research has shifted focus towards the direct control of robots through LLM-driven code generation. The `Code-as-policies '~\cite{code-as-policies} paradigm has showcased remarkable zero-shot capabilities across diverse tasks. Theoretically, it could serve as a viable solution for the semantic rearrangement problem, given the proficiency of LLMs in comprehending pattern compositions and inferring object selections from linguistic cues. 

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{Pictures/robot_setup.jpg}
    \caption{\small{Robot Setup. We use a UR5e robot equipped with a RealSense D455 camera.}}
    \label{fig:robot}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth, height=3cm]{Pictures/config.png}
    \caption{
    \small{Illustration of infeasible start and goal configuration. In this scene, block 2 is in an infeasible start configuration. And the goals of blocks 3 and 2 are infeasible without an excessive
number of intermediate steps.}}
    \label{fig:infeasible-config}
    \vspace{-0.5cm}
\end{figure}
Current methods such as StructFormer and Code-as-policies often fail to produce collision-free arrangements, whereas StructDiffusion incorporates a learning-based collision checker. However, collision-free does not mean executable, as shown in Fig.~\ref{fig:infeasible-config}. For example, block 3 obstructs block 2's target position, complicating block 1's motion. This highlights the challenge of distinguishing between collision-free and executable goals, as some may be the former but not the latter, or may require excessive steps to execute.

% Despite their capabilities, current methods face challenges when deployed in real-world scenarios. These methods do not always guarantee executable outcomes from their plans. Both StructFormer and Code-as-policies fall short in generating collision-free goal arrangements. On the other hand, StructDiffusion incorporates a learning-based collision checker to yield a collision-free goal arrangement. However, it is important to distinguish between a collision-free goal arrangement and an executable plan. As illustrated in Fig.~\ref{fig:infeasible-config}, a goal configuration may be collision-free yet still inexecutable. Consider block 2, for instance: the initial movement of block 1 depends on block 1's movement. Additionally, block 3 already occupies block 2's intended goal position. This underscores the inherent challenge in separating planning and arrangement goal generation: some goals might align with the language description and be collision-free, but they might also be unexecutable or necessitate an excessive number of steps for execution.



% Key insights: we model it as a sequential sampling problem.
% This study introduces \textbf{LGMCTS} for executable semantic object rearrangement. 
This study presents the \textbf{L}anguage-\textbf{G}uided \textbf{M}onte-\textbf{C}arlo \textbf{T}ree \textbf{S}earch (LGMCTS) technique,  designed specifically for executable semantic object rearrangement. LGMCTS leverages LLMs to interpret free-form language and consider object placements as probability distributions, not exact points. We frame the challenge as a sequential sampling problem, where each object's pose is drawn from a distribution influenced by language and the current scene state. The approach incorporates distracting objects, enabling plans that meet language criteria while also being executable.

% This study presents the \textbf{L}anguage-\textbf{G}uided \textbf{M}onte-\textbf{C}arlo \textbf{T}ree \textbf{S}earch (LGMCTS) designed specifically for executable semantic object rearrangement. LGMCTS seamlessly integrates the prowess of LLMs in understanding free-form language descriptions while acknowledging that such descriptions typically suggest regions rather than exact points for objects. Given that each object's pose correlates with a probability distribution hinted at by the language, we reinterpret the semantic rearrangement challenge as a sequential sampling endeavor. In each iteration, an object's position is derived from a pose distribution shaped by linguistic cues and the current scene configuration. By integrating distracting objects into this sequential sampling approach, we can craft a plan that not only aligns with the language criteria but is also executable.

The primary contributions of this study are: 1) Introducing a novel approach that concurrently addresses semantic rearrangement goal generation and action planning 2) Presenting a unique method that facilitates zero-shot multi-pattern composition for semantic object rearrangement 3) Establishing a new benchmark tailored for executable semantic object rearrangement.
% % Key contribution
% In contrast to existing approaches for semantic rearrangement, LGMCTS stands out by seamlessly handling multi-pattern compositions, accommodating free-form language inputs, and addressing both the starting and goal configuration dependencies within a singular framework. We provide a quantitative assessment of LGMCTS using simulation data and offer a qualitative evaluation employing the UR5e robot in multiple intricate real-world scenarios.
% Overall structure

==> introduction_long.tex <==
\section{Introduction}
Everyday tasks, such as ``Set up the kitchen", involve organizing objects based on verbal instructions, a process that is intuitive for humans but that presents a significant challenge for robots. The semantic rearrangement problem seeks to empower robots with the ability to reorganize a scene according to linguistic descriptions. This challenge necessitates that robots comprehend the task through natural language, and address the corresponding Task And Motion Planning (TAMP) problem effectively.

Traditionally, solving this problem requires formalizing the semantic rearrangement issue into a symbolic representation, clearly defining the goal configuration or constraints. Subsequently, one can employ formal planners such as STRIPS~\cite{fikes1971strips} (Stanford Research Institute Problem Solver) and PDDL~\cite{aeronautiques1998pddl} (Planning Domain Definition Language), or search-based planners like MCTS (Monte-Carlo Tree Search) to devise a feasible plan. While this approach can yield optimal and complete solutions, it demands expert-level knowledge to abstract a specific problem into a formal representation, making it less accessible to the average user.

To overcome this challenge, numerous recent studies have sought to tackle the problem directly from linguistic inputs and RGB-D observations~\cite{clip_port,struct_diffusion,liu2022structformer}. One approach uses multi-modality transformers to establish a correlation between verbal descriptions and object positions using data generated from the simulation. Following work such as StructDiffusion~\cite{struct_diffusion} further improved this method by using a diffusion model to build the multi-modality solution. However, a common drawback of these methods is that they rely on an offline training stage, which makes them applicable only to trained object categories and spatial patterns.

\begin{figure}
    \centering
    \includegraphics[width=0.65\linewidth]{Pictures/robot_setup.jpg}
    \caption{\small{Robotic Setup: a UR5e robot equipped with a RealSense D455 camera. The task is to re-arrange the objects, which are unknown to the robot, according to a natural language instruction.}}
    \label{fig:robot}
\end{figure}

With the advent of Large Language Models (LLMs), models such as GPT~\cite{gpt3} and Llama~\cite{llama2, llama} have demonstrated impressive potential in understanding complex scenarios and exhibiting zero-shot planning capabilities. This has led researchers to explore the utilization of LLMs in solving language-based TAMP problems. One pioneering study, utilizing LLM as a zero-shot planner~\cite{huang2022language}, employed GPT-3 to generate a sequence of text-based sub-steps, while integrating the sub-steps with a set of predefined skills. Following this, SayCan~\cite{ahn2022can} delved into addressing the feasibility of plans generated by LLMs by combining LLMs with a learned feasibility estimator~\cite{ahn2022can}. Subsequently, Code as Policies~\cite{code-as-policies} leveraged a blend of LLMs and action-APIs, showcasing impressive zero-shot performance across a broad spectrum of tasks. However, despite specific considerations for the feasibility of plans proposed by LLMs, it has been reported that these plans significantly lag in executability and completeness when compared to those crafted by a properly implemented traditional solver designed for the task~\cite{valmeekam2022large}. This observation has naturally led researchers to seek methods that merge the user-friendliness of LLMs with the robustness of traditional TAMP algorithms such as PDDL, STRIPS, or MCTS. LLM-GROP~\cite{ding2023task} first tries this approach in rearrangement, employing LLMs to parse user tasks from language into pairwise spatial relationship specifications and then call a sampling-based task and motion planner~\cite{zhang2022visually} to generate the plan. The limitation of LLM-GROP is that it can only handle pair-wise relationships, and thus it cannot perform complex rearrangement tasks.
AutoTAMP~\cite{chen2023autotamp} uses LLMs to translate natural language into formal representations, and then invokes a planner to tackle the problem. AutoTAMP can solve a wide range of TAMP tasks, but it does not apply to general semantic rearrangement where the action space is not discrete and potentially large.

% With the advent of Large Language Models (LLMs), models such as GPT-4 and Llama2 have demonstrated significant potential in understanding complex scenarios and exhibiting zero-shot planning capabilities. This has led researchers to explore utilizing LLMs in solving language-based TAMP problems, with innovations like AutoTAMP using LLMs to parse natural language into formal representations, thereby combining the accessibility of LLMs with the robustness of traditional TAMP algorithms. More recently, the development of LLM-GROP has brought the AutoTAMP approach into the object rearrangement setting, employing LLMs to parse user tasks from language into pairwise spatial relationships specifications and then call a rule-based planner to generate the plan. However LLM-GROP is limited only to pairwise spatial relationship and due to its separate handling of task planning and motion planning, its plan may not be optimal for execution.

We present Language-Guided Monte-Carlo Tree Search (LGMCTS), a new algorithm for executable semantic object rearrangement. Like its predecessors, AutoTAMP and LLM-GROP, LGMCTS leverages LLMs for generating intermediate representations and employs a planner for formulating feasible plans. A key novelty of LGMCTS is the integration of parametric geometric priors for spatial relationship representations. LGMCTS facilitates more nuanced handling of complex geometric relationships among multiple objects, addressing scenarios that require organization beyond simple pairwise interactions, such as configurations in lines or rectangles. Additionally, LGMCTS takes a holistic approach by simultaneously considering task planning (goal specification) and motion planning (execution order and intermediate steps). During planning, an obstacle relocation strategy is used to handle obstacles that may block the execution.
This coordination ensures that plans are not only semantically coherent but also practically executable, offering a balanced consideration of goal achievement and operational efficiency.

To assess the efficacy of LGMCTS, we introduce the Executable Language-Guided Rearrangement (ELGR) benchmark, featuring over 1,600 varied language queries and robot execution checks. Our evaluations indicate that LGMCTS performs effectively on the ELGR benchmark, especially in comparison with Code as Policies and Progprompt in terms of feasibility and semantic consistency of the generated goals. LGMCTS also outperforms Structformer and StructDiffusion in goal generation  on the Structformer dataset.

% % Semantic Rearrangment
% In daily life, tasks like ``Set up the kitchen" require arranging objects according to language cues, an intuitive process for humans but a complex challenge for robots. The semantic rearrangement problem aims to enable robots to reconstruct scenes based on linguistic descriptions. Such problem requires the robot to understand the problem from natural language and solving the corresponding Task And Motion Planning (TAMP) problem.

% % Tranditional Task and motion planning, lack of user-frientdly interface, senstive to variable numebers.
% % Consider the task: ``Set the dinnerware for dinner and place a candle in front of a plate." A robot must identify the items constituting `dinnerware' and their correct arrangement, while also handling real-world constraints like initial object coverings and spatial obstacles. The command introduces two key constraints: 1) `dinnerware' must be arranged appropriately for dinner, and 2) a candle must be placed in front of a plate. This example highlights the problem's complexity.
% Traditionally, to solve such problem, we need to formalize the semantic rearrangement problem into a symbolic representation and clearly claim the goal configuration or constraints. Then we can call formal-planner such as DDPL, STRIPS or search-based planner, MCTS to provide a feasible plan. Although such method can be optimal and complete, it requires expert level knowledge to abstract a specific problem to a formal representation, which makes it unfriendly to common user.

% % Approaches-1: Multi-modality transformer
% % Structformer, VIMA, CLIPPORT
% To address this limitation, there are many new works trying to address this problem directly from language input and RGB-D observation. One approach employs a multi-modality transformer~\cite{clip_port, liu2022structformer, vima} to learn the mapping between language and object poses through simulated arrangements and rule-based language descriptions. However, this method has limitations. It assumes that language descriptions map to precise ground-truth poses, which is often unrealistic. It is also less adaptable to free-form linguistic inputs, as it performs best with descriptions similar to its training data. Recent research employs diffusion models to capture how language tokens map to spatial distributions. DALL-E-Bot~\cite{Dall-e-bot} uses text-to-image to generate target images and derive poses, while StructDiffusion~\cite{struct_diffusion} employs a diffusion model conditioned on language and point-cloud embeddings. Both approaches show promise but have limitations: DALL-E-Bot can be unstable and distracted by extraneous objects, whereas StructDiffusion is constrained to known training patterns and lacks zero-shot adaptability.

% % LLM is easy to use but feasiblity can be a problem.
% With the rise of Large Language Model (LLM), models such as GPT-4 and LAMA-2 has shown great potential in dealing with complex scenario understanding and zero-shot planning ability. Researchers begin to investigate how to unitize LLM to solve the language-based TAMP problem. Language model as zero-shot planner~\ref{huang2022language} is one of the first work using LLM in TAMP. It uses GPT-3 to generate a series of text-based sub-steps and then combine it with a series of pre-defined skills. SayCan further investigate the feasibility problem for the plan generated by LLM through combing LLM with a learned feasibility estimator~\ref{ahn2022can}. Later Code-as-policies~\cite{code-as-policies} uses a combination of LLM and action-API and show a good zero-shot performance on a wide range of tasks. However even with a specific consideration on the feasibility of LLM proposed plan, it is reported the plan generated by LLM is significant worse in terms of success rate and completeness compared with 
% a proper implemented traditional solver tailored for the task~\cite{valmeekam2022large}. Naturally, researchers start to looking for a way to combine the easy-to-use of LLM and the completeness of traditional TAMP algorithm such as TDDL, STRIPS, or MCTS. Instead of directly generating a solution using LLM, AutoTAMP~\cite{chen2023autotamp} tries to use LLM to parse natural language to formal representation, and then call formal-planner to solve it, providing an paradigm in combing LLM and traditionally planner family.

% More recently, LLM-GROP brings such AutoTAMP fashison into object-rearrangment setting, where they use LLM to parse user's task from language to pair-wise spatial relationship and use a sampling\& rejection to generate the goal specification. Then they use a rule-based planner to generate feasible plan. This approach has two limitations, 1. their modeling can only consider pair-wise object relationship, and can not be generalized to patterns where requires multiple objects, such as lines or rectangles. 2. In their modeling, goal generation and action plan are generated separately. So their generated goal may be the best for acting.

% We present Language guided Monte-Carlo Tree Search, an algorithm for executable semantic object rearrangment. Similar to AutoTAMP and LLM-GROP, we also use LLM to generate intermediate representation and call an planner to provide a feasible plan. There are two major differences. Instead of using pair-wise spatial relationship, LGMCTS introduce parametric geometric priors as spatial relationship representation, which provides us with the ability to deal with more complex geometric relationship between multiple objects. Secondly, in LGMCTS, we simultaneously consider the task planning (goal specification) and motion planning (execution order and intermediate steps). Such joint consideration enable LGMCTS to generate more efficient solution while fitting to the semantic constraints. As for evaluation, we find there lacks an massive quantitive evalution benchmark for executable semantic rearrangment. Existing benchmark such as Structformer only evaluates on wheather generated solution meets the constraints and is collision-free. However, the collision-free goal specification is not always executable as we demonstrated in Fig. To better quantitatively evaluate the success rate and efficiency of different algorithm on semantic re-arrangement, we introduce ELGR with 2,000 different language queries and robot execution checking. We demonstrate the effectness of LGMTCS on ELGR benchmark. We also compare with two previous transformer-based and diffusion-based method, Structformer and StructDiffusion on Structformer dataset on the quality of generated goal.


==> proposed-new.tex <==
\section{Method}
\label{sec:method}
In a nutshell, LGMCTS starts by calling an LLM to parse the language description $L$ to a list of spatial distributions $\mathcal{F}=\{f_i: p(o_i) \sim f_{i} | o_i \in O_R\}$. Then it uses an MCTS-based procedure to find a physically feasible action sequence $A$ to rearrange the scene according to distributions $\mathcal{F}$.

\subsection{Language Parsing \& Object Selection} \label{sec:parse}
During the language parsing stage, we parse $L$ into $\mathcal{F}=\{f_i: p(o_i) \sim f_{i} | o_i \in O_R\}$. Similar to previous methods~\cite{code-as-policies}, we conduct an automated prompt engineering to guide the LLM to perform the parsing. Fig.~\ref{fig:llm_parsing} showcases how prompt engineering is implemented. Essentially, the language model translates user requirements into structured goal configurations and constraints that guide task execution.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{Pictures/icra_listing-drawio.png}
    \caption{\small{An example of language parsing. We are using GPT-4~\cite{gpt3} in this work.}}
    \label{fig:llm_parsing}
\end{figure}

Consider the example depicted in Fig.~\ref{fig:llm_parsing}. First comes the {\bf system prompt} providing guidelines for the LLM to follow when interpreting user queries. Then, we need to provide an {\bf object description} such as semantic labels, colors, and IDs for the objects in the scene. In practice, we use the Recognize Anything Model (RAM)~\cite{huang2023tag2text, zhang2023recognize} for producing the semantic labels, and a color detector to determine the colors of the objects in the scene. A unique ID is assigned to each object. Finally, we provide a {\bf user query} describing the rearrangement goal. A structured answer is returned from the LLM.
LLM's answers suggest how many patterns there are and which objects should be selected to form the pattern.

\subsection{Parametric Geometric Prior} 
\label{sec:prior}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Pictures/prior.png}
    \caption{\small{Visualization of $(x,y)$ prior for `line' pattern. From left to right: $K=0$, $K=1$, $K=2$, $K=3$, where $K=|O_{R}^{sampled}|$, the number of sampled object poses. White star marks are sampled poses. When $K=0$, the pose can be sampled anywhere. When $K=1$, it needed to sampled outside a circle region. After that, all poses will be sampled along the line defined by the first two poses. }}
    \label{fig:prior}
\end{figure}

As mentioned in Section~\ref{sec:problem}, if we know the goal position distribution for each object, the semantic rearrangement problem can be converted to a sequential sampling problem. There are multiple details we need to pay attention to in this process. (1) The position distribution is not fixed but varies with the progress of sampling. For example, if we say objects A, B, and C need to be put into a line, and we sample in the order of A, B, and C, then the distributions of A and B are actually unbounded, and C must be placed on the line defined by the positions of A and B. (2) The position distribution should be collision-free. (3) One can build a database for many different spatial distributions, but we need to have a flexible mechanism to associate LLM's inferred distribution types with items in the database.

We show in the following how to compute the pose distribution function \( f_{i}(p_i|P_S, L) \) for each object  \( o_i \) in the set \( O_R \) during the sequential pose sampling process. Here, \( p_i \) denotes the pose \((x, y, \theta)\) of an object \( o_i \), \( P_S \) represents the list of current poses for all objects in the scene, and \( L \) is the natural language command. 

We compute \( f_{i}(p_i|P_S, L) \) as an element-wise product of two components, a pattern prior function \( f_{\text{prior}}(p_i|P_{R}, L) \) and a boolean function \( f_{\text{free}}(p_i|P_S) \) of the workspace,
\begin{equation}
    f_{i}(p_i|P_S, L) = f_{\text{prior}}(p_i|P_{R}, L) \times f_{\text{free}}(p_i| P_S)
\end{equation}
In this equation, \( P_{R} \) \color{blue} is the list of current poses of all objects in  \( O_{R} \)\color{black}. 
\color{blue}
We note that \( P_{R} \) is a subset to \( P_{S} \).
\color{black}
The function \( f_{\text{free}}(p_i|P_S) \) is set to $1$ \color{blue} if $p_i$ is collision-free from the remaining poses in $P_S$, and to $0$ otherwise. \color{black} $f_{\text{free}}$ is determined by running a 2D collision simulation using point cloud observations for each object \( o_i \) \(\in\) \( O_S \).

Our primary focus is to determine \( f_{\text{prior}}(p_i|P_{R}, L) \). To this end, we employ an approach akin to the one described in \cite{ahn2022can}. We maintain a database comprising a collection of predefined prior functions. Each of these functions is linked with one or more Sentence-BERT embeddings, acting as keys. The function corresponding to the best matching key is selected, as follows,
\begin{equation*}
     f_{\text{prior}}(p_i|P_{R}, L) = f_{\text{prior}}^K(p_i|P_{R}) \textrm{ with } K = \underset{K\in \text{database}}{\text{argmax}}(\Theta_k \cdot \Theta({L}))
\end{equation*}
Here, \( \Theta_k \) is the \( K^{th} \) key in the database, and \( \Theta({L}) \) is the Sentence-BERT embedding generated from the language instruction \( L \).
In summary, the most suitable prior function from the database is selected based \color{blue} on \( \Theta({L}) \) \color{black}.


We now delve into the definition of \( f_{\text{prior}}^K(p_i|P_{R}) \) in the context of our work. We use a unique model for representing various distributions by employing parametric curves. A parametric curve can be expressed as \( (x, y) = \gamma(t, \kappa) \), where \( t \) ranges from 0 to 1 and \( \kappa \) is a set of curve-defining parameters. In our work, \( \kappa \) is modeled as a function of two 2D positions, denoted as \( \kappa(p_0, p_1) \). Therefore, for each pattern, we define two functions: \( \gamma \) and \( \kappa \).

Given that pattern prior $f_{prior}$ is used inside a sequential sampling process (check Section~\ref{sec:mcts} for more details), the prior distribution needs to be iteratively updated to capture the history of sampling. Consequently, we further categorize \( O_{R} \) 
% (the subset of objects involved in given instruction $L$) 
based on whether the objects have been sampled in the current branch of the MCTS-Planner. Subsets \( O_{R}^{sampled} \) and \( O_{R}^{unsampled} \) denote the sampled and non-sampled objects, respectively. Thus, $O_{R} = O_{R}^{sampled} \cup O_{R}^{unsampled}$.

The probability  \color{blue} $f_{\text{prior}}^K(p_i|P_{R}))$ \color{black} of sampling a pose $p_i = (x_i, y_i, \theta_i)$ for next object \color{blue} $o_i\in O_{R}^{unsampled}$ \color{black} is given as follows.
\begin{itemize}
    \item If \color{blue} $|O_{R}^{sampled}|=0$ \color{black} then \( (x_i, y_i, \theta_i) \sim U \), suggesting that the first object can be placed arbitrarily.
    \item If $|O_{R}^{sampled}|=1$ then \( \sqrt{(x_i - x_0)^2 + (y_i - y_0)^2} \leq \delta \) and \( (x_i, y_i, \theta_i) \sim U \), imposing that the second object must be sampled uniformly at a position that is distanced from the first by at most \( \delta \).
    \item If $|O_{R}^{sampled}|>1$ then \( (x_i, y_i) = \gamma\big(\frac{|O_{R}^{sampled}|}{|O_{R}|}, \kappa(p_0, p_1)\big) + \epsilon \) where \( \epsilon \sim G(0, \sigma) \), here $G$ represents a Gaussian distribution \color{blue} with mean zero \color{black} and variance $\sigma$, \color{blue} and \color{black}  $\theta = atan2(1, \gamma'(\frac{K}{N}))$. \color{blue}For $\theta$, \color{black} we use the angle of gradient represented as the rotation angle of the object.
\end{itemize}

Our parametric geometrical representation enables us to model any geometric shapes that can be written into the format of a parametric curve. In our current implementation, we defined shapes such as ``line," ``circle," ``rectangle," ``tower," ``spatial:left," ``spatial:right" and so on. Due to space constraints, we refrain from elaborating on the definitions of $\gamma$ and $\kappa$ for all these predefined patterns.  Fig.~\ref{fig:prior} illustrates an example of a parametric geometric prior. Noticeably, we divide patterns into ``ordered" and ``unordered" based on whether the pattern requires an execution sequence.

Note that in our work, language instruction $L$ is typically composed of multiple instructions that deal with different subsets of objects. Specifically, $L$ can be interpreted as a list \color{blue} $\{L_i\}_{i=1}^k$ of sub instructions $L_i$ \color{black}. For example, an instruction $L$ can be a composite instruction: $L = \{L_1, L_2\}$, where $L_1$ refers to placing objects $A$, $B$, and $C$ in a line, and instruction $L_2$ refers to placing object $A$ on the left of $B$. Each language instruction $L_i\in L$ is associated with a subset of objects \color{blue} $O_{R_i} \subseteq O_R$\color{black}. In our example, $O_{R_1} = \{A,B,C\}$ and $O_{R_2} = \{A,B\}$. In the sequential sampling process described above in this section, we only presented the case of a single language instruction for simplicity, but the same process is used for sampling poses given by a complex instruction. 


\subsection{Monte-Carlo Tree Search (MCTS) for TAMP}  % KAI
\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{Pictures/illustration.png}
    \caption{\small{
A minimal example illustrates our MCTS-Planner's aim to arrange a table. The language description provided is: ``Can you please put the apple behind the spoon? And I also want the cup at the right of the apple." The top row displays the current scene arrangement, while the bottom row shows the $f_{prior}$ and $f_{free}$ for the object being manipulated. $f=f_{prior} \times f_{free}$. In the probability figure, black represents 0, and white represents 1.
}}
    \label{fig:mcts_exmp}
\end{figure}
\label{sec:mcts}
As previously mentioned, our rearrangement problem can be formulated as a sequential task. In each step, we sample a pose $p_i$ for each object \color{blue} $o_i \in O_R$ \color{black} according to a pose distribution $f_{i}$ selected by the LLM and computed as described in Section~\ref{sec:prior}. Once we complete all samplings, all objects will have been placed in their desired locations. However, this task cannot be executed by the robot in a naive sequential order, as the rearrangements made in previous steps may obstruct subsequent sampling. Therefore, we propose a task and motion planner based on the Monte Carlo Tree Search (MCTS) algorithm to simultaneously arrange the task and address object relocation issues. The objective of our MCTS-Planner is to fulfill all object position requirements defined by $\mathcal{F}$, the spatial distribution list. In the MCTS-Planner, we maintain a tree where each node $s$ in the tree comprises the current objects' poses, $\{p_1, p_2, ..., p_N\}$, and the remaining object spatial requirements $\mathcal{F}_r$, where $\mathcal{F}_r \subseteq \mathcal{F}$.

Formally, the MCTS-Planner is structured into four phases: selection, expansion, simulation, and back-propagation, as detailed in Section~\ref{sec:mcts_frame}. The selection, expansion, and back-propagation stages follow the methodology outlined by \cite{labbe2020monte}. The reward for transitioning to a new state $s$ is quantified by the reduction in the number of spatial requirements, that is, $|\mathcal{F}|-|\mathcal{F}_r|$. This reward structure mirrors the approach in \cite{labbe2020monte}, aiming to steer the search towards branches that efficiently move objects to their goal poses. The simulation phase is elaborated in Algorithm~\ref{alg:Simulation}. This phase begins with the MCTS state $s$ and an attempted action of placing an object $o_i$ in a pose $p_i\sim f_i$, where $f_i$ is the pose distribution explained in the previous section. If the targeted object $o_i$ is not reachable, e.g. there exist some obstacles above it, a reachable obstacle is randomly selected from those above it, and a collision-free pose within the workspace is sampled for relocation (Lines 2-5). If $o_i$ is reachable, an attempt is made to sample its pose with distribution $f_i$ (Line 7). \color{blue} If the sampled pose is not collision-free, we will randomly choose an obstacle in the collision and relocate it to \color{black} a collision-free pose within the workspace (Lines 9-13).
Note that obstacle relocation may add previously placed objects back to the requirement list $\mathcal{F}_r$.
However, this obstacle relocation strategy increases the robustness of our rearrangement planner, especially when the environment is cluttered.
Although MCTS operates as an anytime search algorithm, our MCTS-Planner implementation returns the first solution it finds. Furthermore, we have proved that the MCTS-Planner is probabilistically complete within our specified framework in Proposition~\ref{prof:mcts}.

Fig.~\ref{fig:mcts_exmp} presents an illustrative example of the MCTS-Planner at work. Owing to space constraints, we will only explore three simulation steps along the branch that yield a feasible solution. In this scenario, the user requests, ``Can you please put the apple behind the spoon? And I also want the cup to be at the right of the apple." In response, the LLM generates the spatial distribution list $\mathcal{F}=\{f_1, f_2\}$, where $f_1$ is for positioning the apple behind the spoon, and $f_2$ is for placing the cup to the right of the apple. Fig.~\ref{fig:mcts_exmp}(a) illustrates the initial arrangement of objects. Given the dependency of $f_2$ on the apple's position, $K$ actions will be sampled for $f_1$, but none for $f_2$ in this initial setup. Fig.~\ref{fig:mcts_exmp}(b) depicts the outcome of an action of sampling a pose from $f_1$, where the apple is relocated according to $f_1$. The dashed-line circles represent the other $K-1$ actions originating from the root node. After sampling $f_1$, we are left with $\mathcal{F}_r=\{f_2\}$ as shown in Fig.~\ref{fig:mcts_exmp}(b), and an attempt is made to position the cup to the right of the apple. However, the goal position is in collision with the knife, so we need to relocate the knife. Fig.~\ref{fig:mcts_exmp}(c) demonstrates the knife's relocation, maintaining $\mathcal{F}_r=\{f_2\}$. Ultimately, Fig.~\ref{fig:mcts_exmp}(d) showcases the final planning result.


\begin{algorithm}
\begin{small}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwComment{Comment}{\% }{}
    \caption{Simulation}
		\label{alg:Simulation}
    \SetAlgoLined
		\vspace{0.5mm}
    \Input{$s$: an MCTS state,\\ 
    $f_i$: a pose distribution {\footnotesize (place $o_i$ in a pose $p_i\sim f_i$)}.
    }
    \Output{$(o,p)$: a rearrangement action {\footnotesize (place $o$ in pose $p$)}.}
\vspace{0.5mm}

\If{$o_i$ is not reachable}
{
Select a reachable object $o$ that is blocking object $o_i$;\\
$p\gets$uniformSampling($o,s$);\\
\lIf{$p$ exists}{\Return ($o$,$p$)}
\lElse{\Return \textbf{failure}}
}
\Else{
$p\gets$sampling($o_i, s, f_i$);\\
\lIf{\text{collisionFree$(o_i,p,s)$}}{\Return ($o_i$,$p$)}
\Else{
$o \gets$ Randomly choose an obstacle in collision;\\
$p\gets$\text{uniformSampling$(o,s)$};\\
\lIf{$p$ exists}{\Return ($o$,$p$)}
\lElse{\Return \textbf{failure}}
}
}

\end{small}
\end{algorithm}

\begin{proposition}\label{prof:mcts}
MCTS-Planner is probabilistic complete.
\end{proposition}
\begin{proof}
For a semantic rearrangement task and the distribution list $\mathcal{F}$, assume that there is a feasible action sequence $A^*$ moving objects to a final arrangement $A_f$, such that $f_{i}(A_f[o_i]) > 0 \ \forall o_i\in O_R$.
Denote p as the probability that MCTS can find an action sequence satisfying the goal state criteria. We prove $\lim_{K \to \infty} p=1$.

First, we prove that there is an action sequence $A^*_0$ whose actions can all be generated by MCTS-Planner.
Note that in MCTS-Planner, an action satisfies either of the two rules: \textbf{R1}: Move an object $o_i$ to goal: it requires $o_i\in O_R$ and the new pose $p$ satisfies goal pose requirements (i.e., $f_i(p)>0$); \textbf{R2}: Obstacle relocation: the old pose $p$ of the moved object makes other objects not reachable or it lies in others' goal regions, i.e., $\exists f\in\mathcal F_r, \ s.t. f(p)>0$ (Line 2, 10).
We construct $A^*_0$ by reordering and deleting actions in $A^*$ as follows: (1) If an action in $A^*$ satisfies \textbf{R1} or \textbf{R2}, we add the action to $A^*_0$. 
Otherwise, we delay the addition until it satisfies the rules; 
(2) If the action still cannot satisfy the rules before we examine the next action in $A^*$ for the same object, we delete the former action. 
Thus, all the actions in $A^*_0$ can be generated by MCTS-Planner, and the final arrangement is $A_f$.

Next, we prove that the probability for MCTS to find an action sequence in the ``neighborhood'' of $A^*_0$ approaches 1 as $K$ increases. 
For each intermediate state $s$ of $A^*_0$, denote $(A^*_0[s].o, A^*_0[s].p)$ the rearrangement action that $A^*_0$ chooses at $s$.
Let $r:=(\min_{1 \leq i\leq |A^*_0|} C_i)/2|A^*_0|$, where $C_i$ is the minimum distance making the placement pose of the $i^{th}$ action of $A^*_0$ invalid (out of goal distribution or in collision).
For an intermediate state $s$ of $A^*_0$, let $p_r^s$ be the probability that after $K$ actions, there is an action moving $A^*_0[s].o$ to the $r-$neighborhood of $A^*_0[s].p$.
We have
$$
    \lim_{K \to \infty} p \geq \lim_{K \to \infty} \prod_{s\in A^*_0}p_r^s \geq \lim_{K \to \infty} (1-(1-\dfrac{\pi r^2}{| W| N})^K)^{|A^*_0|}
$$

where $|W|$ is the size of the workspace. Specifically, the second function indicates the probability of finding a feasible action sequence, where the intermediate state object poses are maintained in the neighborhood of those in $A^*_0$.
In the third function, 
$(\pi r^2)/(|W|N)$ is the lower bound of the probability of choosing an action in $s$, moving $A^*_0[s].o$ to the $r-$neighborhood of $A^*_0[s].p$ and the base of the $|A^*_0|$ exponent is a lower bound of $p_r^s$.
Since $K$ is the only variable in the third function, $\lim_{K \to \infty} p=1$.
\end{proof}

